StrNim: a variant of Nim played on strings

We propose a variant of Nim, named StrNim. Whereas a position in Nim is a tuple of non-negative integers, that in StrNim is a string, a sequence of characters. In every turn, each player shrinks the string, by removing a substring repeating the same character. As a first study on this new game, we present some sufficient conditions for the positions to be P-positions.

==> docs/acknowledgement.tex <==
\section{Acknowledgement}
